Don't Trade Off Safety: Diffusion Regularization for Constrained Offline RL

Constrained reinforcement learning (RL) seeks high-performance policies under safety constraints. We focus on an offline setting where the agent has only a fixed dataset -- common in realistic tasks to prevent unsafe exploration. To address this, we propose Diffusion-Regularized Constrained Offline Reinforcement Learning (DRCORL), which first uses a diffusion model to capture the behavioral policy from offline data and then extracts a simplified policy to enable efficient inference. We further apply gradient manipulation for safety adaptation, balancing the reward objective and constraint satisfaction. This approach leverages high-quality offline data while incorporating safety requirements. Empirical results show that DRCORL achieves reliable safety performance, fast inference, and strong reward outcomes across robot learning tasks. Compared to existing safe offline RL methods, it consistently meets cost limits and performs well with the same hyperparameters, indicating practical applicability in real-world scenarios.

==> file/3_method.tex <==

\section{Methodology}


\subsection{Diffusion Model for Policy Extraction}
Our main idea is to fully exploit the offline dataset to obtain a behavioral policy, and use the behavioral policy to guide the training of the target policy. A policy $\pi(a\vert s)$ is  a distribution on the action space. Previous work estimated the behavior policy with  maximum likelihood estimation \cite{fujimoto2021minimalist} or leveraged a conditional variational autoencoder \cite{kingma2013auto,sohn2015learning}. Here, we exploit the concept of diffusion models \cite{sohl2015deep,ho2020denoising,song2020score} to learn the unknown behavioral policy $\pi_b(a\vert s)$ given its strong generative capabilities. Diffusion models have emerged as powerful generative tools to generate data sample $x_0\sim p(x_0)$ with few-shot samples. They work by using a forward process $q(x_{t}\vert x_{0})$ to perturb the original distribution to a known noise distribution. Subsequently, this model generates the samples using the reverse denoising process $p_{\psi}(x_{t-1}\vert x_t)$.  The forward process can generally be written with a forward stochastic differential equation (SDE)
\begin{equation}
    dx = -\frac{\beta(t)}{2}xdt + \sqrt{\beta(t)} dW_t, \label{forward sde}
\end{equation}
where $\beta(\cdot): [0,T]\rightarrow \R^+$ is a scalar function and the  process $\{W_t\}_{t\in [0,T]}$ is a standard Brownian motion. Our forward process is the discretized version of SDE in Eq.~(\ref{forward sde}) perturbing the original distribution to Gaussian noise. For example, if we choose a variance preserving SDE for the forward diffusion process as in \cite{ho2020denoising}, each step $x_t$ is perturbed with the noise $z_t\sim \mathcal{N}(0,I)$ to obtain $x_{t+1} = \sqrt{\alpha_t}x_t+ \sqrt{\beta_t} z_t$, where $\beta_t = 1-\alpha_t \in (0,1)$. We denote $\Bar{\alpha}_t = \prod_{i=1}^{t}\alpha_i$ and $\Bar{\beta}_t = 1-\Bar{\alpha}_t$. Therefore,  we can rewrite $x_t = \sqrt{\Bar{\alpha}_t}x_0 + \sqrt{\Bar{\beta}_t} \epsilon_t$, where $\epsilon_t\sim \mathcal{N}(0,I)$ follows the standard Gaussian distribution.  The reverse denoising process is optimized by maximizing the evidence lower bound of the log-likelihood $\E[\log p_{\psi}(x_0)]$  defined as $\E_{q(x_0:x_{T})}\big[\log \big(p_{\psi}(x_{0:T})/q(x_{1:T}\vert x_0)\big)\big]$. We can then rewrite the loss function into the weighted regression objective in Eq.~(\ref{weighted regression}) and transform the problem into training a denoising function  $\epsilon_\psi$ predicting the Gaussian noise $\epsilon_t$:
\begin{equation}
   \hspace{-5pt}\mathcal{L}({\psi}) \hspace{-2pt}= \hspace{-2pt} \E_{t\in \operatorname{Unif}[0,T]}\big[w(t)\|\epsilon_\psi(x_t,t)\hspace{-2pt}-\hspace{-2pt}\epsilon_t\|^2\big], \epsilon_t\hspace{-2pt}\sim \hspace{-2pt}\mathcal{N}(0,I),\hspace{-5pt}\label{weighted regression}
\end{equation}
where $w(t)$ is the weight function.
Then the reversing denoising process can be formulated as $x_{t-1} = \frac{1}{\sqrt{\alpha_t}}\big(x_t-\frac{\sqrt{1-\alpha_t}}{\sqrt{1-\Bar{\alpha}_t}} \epsilon_\psi(x_t,t)\big)+\sqrt{\beta_t}z_t$, where $z_t\sim \mathcal{N}(0,I)$. Using this notion,  we can similarly use the diffusion model to diffuse in the action space $\mathcal{A}$ and sample actions given the current state with the reversing process. In \cite{wang2022diffusion}, the authors learned diffusion policies from the offline dataset using guided diffusion. 
The diffusion policy here is $\pi_{\psi}(a\vert s) = \mathcal{N}(a_T;0,I)\prod_{t=1}^{T}p_{\psi}(a_{t-1}\vert a_t, s)$, where $p_{\psi}(a_{t-1}\vert a_t,  s)$ is a Gaussian distribution with mean $m_{\psi}(a_t,t\vert s)$ and variance $\Sigma_\psi(a_t,t\vert s)$ . 
See also \citet{lu2023contrastive,hansen2023idql}, where diffusion policy is used for inference in policy evaluation. The limitation of these methods is that the diffusion models are slow in inference speed, even under the improved sampling scheme in \citet{song2020denoising,lu2022dpm} the reverse denoising process takes at least 10 steps. Therefore, in this work we mainly use diffusion models for pretraining and learning the behavioral policy $\pi_b$. For state-action pair $(s,a)$ in the offline dataset $\mathcal{D}^{\mu}$, we train our diffusion policy model by minimizing the loss 
\begin{equation}
\hspace{-5pt}\mathcal{L} = \E_{(s,a)\in\mathcal{D}^{\mu} }\E_{t\in \operatorname{Unif}(0,T)}\big[w(t)\|\epsilon_\psi(a_t,t\vert s)-\epsilon_t\|^2\big], \hspace{-5pt}
    \label{diffusion pretrain loss}
\end{equation}
where $a_t = \sqrt{\Bar{\alpha}_t}a  + \sqrt{\Bar{\beta}_t}z$ and $z\sim \mathcal{N}(0,I)$. We  assume that the diffusion model can perfectly learn the behavioral policy $\pi_b$, as shown in \citet{de2022convergence}, due to the fact that the target distribution lies on a compact manifold, the first-order Wasserstein distance between the learned policy and the target policy converges to 0 as the discretization length approaches 0.  

\subsection{Diffusion
Regularization}\label{score regularization}
The work \citet{chen2023score} showed under the offline RL setting that one can train a simple policy using the pretrained critic and diffusion policy imitating the behavioral policy. The key step is to use the reverse KL divergence to regularize the target policy to be close to the behavioral policy. The forward KL is the KL-divergence $D_{\operatorname{KL}}(\pi^*(\cdot\vert s)\| \pi_{\theta}(\cdot\vert s))$ while the reverse KL is $D_{\operatorname{KL}}(\pi_\theta (\cdot\vert s)\| \pi^{*}(\cdot\vert s))$. 
As shown in \citet{chen2023score},  the forward KL leads to mode covering issue while backward KL encourages mode-seeking behavior, although the latter is harder to optimize. Therefore, in this work we also choose the reverse KL for regularization.  We also  constrain our policy family to a simple Gaussian policy class $\Pi:\{\pi_\theta(a\vert s)=\mathcal{N}(a;m_{\theta}(s),\Sigma_\theta(s))\}$. Now, we denote the learned diffusion model's score function as $\epsilon_{\psi}(a_t,t\vert s)$ and the corresponding diffusion policy  as $\mu_{\psi}(a\vert s)$. Then, the reverse KL between the policy $\pi_\theta(a\vert s)$ and the approximated behavioral policy $\mu_\psi(a\vert s )$ can be written as $-\mathcal{H}(\pi_\theta(\cdot\vert s))+H(\pi_\theta(\cdot\vert s), \mu_\psi(\cdot\vert s))$. For Gaussian policy, the first part self-entropy term $\mathcal{H}$ can be directly computed in closed form. For $\mathcal{A}=\R^d$, we have 
\begin{equation}
\begin{aligned}
    \mc{H}(\pi_\theta(\cdot \vert s))& = \int_\mathcal{A} -\log \pi_\theta(a\vert s)\pi_\theta(a\vert s)da\\
    &=  \frac{1}{2}\log(\operatorname{det}(\Sigma_\theta(s))) +  \frac{d}{2}\log(2\pi) 
    + \frac{d}{2}.
\end{aligned}
    \label{self entropy}
\end{equation}
Using the reparameterization trick for Gaussian random variables, we can also rewrite the cross entropy term $H(\pi_{\theta}(\cdot\vert s), \mu_\psi(\cdot\vert s))$ as 
\begin{align}
H(\pi_{\theta}(\cdot \vert s), \mu_\psi(\cdot \vert s)\hspace{-1pt}) 
      &\hspace{-2pt}=\hspace{-2pt}  \E_{\pi_{\theta}(\cdot \vert s)}[-\log \mu_\psi(a\vert s)] \label{reparameterization cross entropy} \\
      &\hspace{-2pt}=\hspace{-2pt} \E_{z\sim \mathcal{N}(0,I)}[-\hspace{-2pt}\log \mu_\psi(m_\theta\hspace{-2pt}+\hspace{-2pt}\Sigma_{\theta}^{1/2}z\vert s)].\notag
\end{align}
Finally, to obtain the gradient with respect to the reverse KL divergence we have 
\begin{align}
     &\nabla_\theta D_{\operatorname{KL}}(\pi_\theta(\cdot\vert s)|| \mu_\psi(\cdot \vert s)) \notag\\
        = &\nabla_\theta H(\pi_{\theta}(\cdot\vert s), \mu_\psi(\cdot\vert s)) - \nabla_\theta \mathcal{H}(\pi_\theta(\cdot\vert s))\label{kl divergence gradient}\\
         = &\E_{z\sim \mathcal{N}(0,I)}\big[-\nabla_a\log \mu_\psi(m_\theta(s)+\Sigma_{\theta}^{1/2}z\vert s)\notag\\
        &\cdot\nabla_\theta(m_\theta(s)+\Sigma_{\theta}^{1/2}z)\big]-\frac{1}{2}\nabla_\theta \log(\operatorname{det}\Sigma_\theta(s)).\notag
\end{align}
The work \citet{song2020score} shows that diffusion models essentially estimate the \textbf{score function}:
\begin{equation}
\nabla_{x}\log p(x_t) \approx  s_{\psi}(x_t,t) = -\frac{1}{\sqrt{\Bar{\beta}_t}}\epsilon_{\psi}(x_t,t).
\label{score function}
\end{equation}
Hence,  we can substitute the denoising function $\epsilon_\psi$ into Eq.~(\ref{kl divergence gradient}) to directly compute the gradient.
\subsection{Safe Adaptation}
To design our algorithm, we define the reward and cost optimization objectives respectively as  follows: 
  \begin{align}
           \hspace{-8pt}\text{Reward:} \max_{\pi\in \Pi} \E_{s\sim \mathcal{D}^{\mu}}\big[&V^{\pi}_r(s)\hspace{-1pt}-\hspace{-1pt} \frac{1}{\beta} D_{\operatorname{KL}}(\pi(\cdot \vert s)|| \pi_b(\cdot\vert s))\big]\label{reward optimization}\hspace{-5pt}\\
       \hspace{-8pt}\text{Cost:} \max_{\pi\in \Pi} \E_{s\sim \mathcal{D}^{\mu}}\big[&V^{\pi}_r(s)- \lambda(V^{\pi}_c(s)-l)\notag\\
       &-\frac{1}{\beta} D_{\operatorname{KL}}(\pi(\cdot \vert s)|| \pi_b(\cdot\vert s))\big].\label{cost optimization}
  \end{align}

We consider the reverse KL divergence term in Eq.~(\ref{reward optimization}) and Eq.~(\ref{cost optimization}) as a regularization term to penalize the policy for deviating too far from the behavioral policy \( \pi_b \). In practice implementation, we use the learned diffusion policy \( \mu_\psi \) to replace \( \pi_b \) and compute the gradient for optimization using Eq.~(\ref{kl divergence gradient}). As discussed in \citet{gu2024balance}, to address the conflict between optimizing reward and cost, it is essential to directly handle the gradient at each optimization step. We also adopt the gradient manipulation idea in \citet{gu2024balance}, but we  do so under the offline setting where we no longer have access to updating our critic with the on-policy data.  The gradient manipulation method can be generally described as follows.  For each step where we need to optimize the reward,  we update our gradient with $\theta \leftarrow \theta +\eta g_r$, and when we need to optimize the cost our gradient is updated with $\theta \leftarrow \theta +\eta g_c$. The gradient manipulation aims at updating the parameter $\theta$ with a linear combination of the two gradients  as $\beta_r g_r + \beta_c g_c$. We can use the angle $\phi:= \cos^{-1}\left(\frac{\langle g_r,g_c\rangle}{\|g_r\|\|g_c\|}\right)$ between the two gradients to judge whether the gradients are conflicting or not, namely if $\phi>90^\circ$ the two gradients are conflicting and otherwise they are not conflicting. 
Especially, the final gradient $g$ is computed  via the rule
\begin{equation}
g =
\begin{cases} 
\frac{g_r+g_c}{2}, & \text{if } \phi \in (0,90^\circ) \\
\frac{g_{r}^{+}+g_{c}^{+}}{2}, & \text{if } \phi \in [90^{\circ},180^\circ],
\end{cases}
\label{gradient manipulation}
\end{equation}
where $g_r^+=g_r - \frac{g_r\cdot g_c}{\|g_c\|^2}g_c$ is $g_c$'s projection on the null space of $g_r$ and $g_c^+=g_c - \frac{g_c\cdot g_r}{\|g_r\|^2}g_r$ is $g_r$'s projection on the null space of $g_c$.  It is also shown in \citet{gu2024balance} that under the assumption of  the convexity of the optimization target, one can ensure monotonic improvement using gradient manipulation. As a result,  here we also employ the gradient manipulation method to update our policy parameter. 
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.7\linewidth]{pictures/algo/safe_policy_figure.pdf}
    \caption{Illustration of the soft switching between safe and unsafe policy regions.}
    % \donghao{Need to refer to this figure in the text.}
    \label{algo-procedure}
\end{figure}
With the procedures outlined above, we present our main algorithm in Algorithm \ref{alg: main algo}, where the safe adaptation step is visualized in Figure \ref{algo-procedure} and detailed in Algorithm \ref{alg: Safe Adapt} given in Appendix \ref{algo extension}. Furthermore, we provide the following theoretical results derived from our algorithm, where the proof is deferred to Appendix \ref{app: proof_proposition}.
\begin{algorithm}[tb]
   \caption{DRCORL}
   \label{alg: main algo}
\begin{algorithmic}
   \STATE {\bfseries Input:} Dataset $\mathcal{D}^{\mu}$, slack bounds $h^+$, $h^-$
  \STATE  Pretrain diffusion model $\epsilon_{\psi}$  
   \STATE Pretrain   $\pi_\theta$ with diffusion model $\epsilon_\psi$
  % \donghao{Index $t$ should not appear here.}
  \STATE
    \textit{// Behavior Cloning}
    \STATE Pretrain   $Q_r^{\pi}$, $Q_c^{\pi}$ 
     \STATE
    \textit{// Pretain critic}
    
    \FOR{each gradient step $t$}
    \STATE  Sample mini-batch $\mathcal{B}=\{(s_t,a_t,s_{t}',r_t,c_t)\}_{t=1}^{|\mathcal{B}|}$ 
    \STATE Update critics for reward and cost 
    % \STATE Update diffusion model $\epsilon_\psi$ with $\mathcal{B}$
    \STATE  $g = \operatorname{SafeAdaptation}(\pi_\theta,\epsilon_\psi, Q^{\pi_\theta}_r,Q^{\pi_\theta}_c,h^+,h^-)$
    \STATE Update $\theta\leftarrow \theta + \eta g$
    
    
    % \donghao{Is this step-size different over periods? (in the proof it is constant)}
   \ENDFOR
\end{algorithmic}
\end{algorithm}

% upper bound, show with theta star not an variable
%how to guarantee the constraint violation

\begin{proposition}[Cost Upper Bound]
\label{cost upper bound}
Assume that the cost function $c:\mathcal{S}\times\mathcal{A}\rightarrow [0,c_{\max}]$ is bounded and non-negative.
Let $\Tilde{\pi}(a \vert s)$ be the output policy of Algorithm \ref{alg: main algo}.
Suppose that there exists $\epsilon_{\text{dist}} > 0$ such that $D_{\operatorname{KL}}(\Tilde{\pi}(\cdot \vert s), \pi_b(\cdot \vert s)) \leq \epsilon_{\text{dist}}$ and $
D_{\operatorname{KL}}(\pi_b(\cdot \vert s), \Tilde{\pi}(\cdot \vert s)) \leq \epsilon_{\text{dist}}$.
Let $\epsilon_{\text{adv}}^{b} = \max_s \mathbb{E}_{a \sim \pi_b(\cdot \vert s)}[A_c^{\Tilde{\pi}}(s, a)]$, where $A_c^{\pi}(s, a)$ is the advantage function under policy $\pi$, defined as: $A_c^{\pi}(s, a) = Q_c^{\pi}(s, a) - V_c^{\pi}(s)$.
Then, it holds that:
\begin{equation}
    V_c^{\Tilde{\pi}}(\rho) \leq V_c^{\pi_b}(\rho) + \frac{(c_{\max}+\gamma \epsilon_{\text{adv}}^b)\sqrt{2\epsilon_{\text{dist}}}}{(1-\gamma)^2}.
\end{equation}
\end{proposition}
This proposition establishes that if the learned policy is constrained to remain within a neighborhood of the dataset’s behavior policy, its safety performance is at least guaranteed to match that of the behavior policy underlying the dataset.
% By regularizing the policy during the learning process with the reverse KL-divergence, assume there exists a constant  such that the distance between $\Tilde{\pi}$ and $\pi_b$ is bounded as follows: .

To theoretically ground our algorithm, we analyze its convergence properties in the tabular setting, where the state and action spaces are finite (i.e., \(|\mathcal{S}|, |\mathcal{A}| < \infty\)). Under softmax parameterization, we derive convergence guarantees when optimizing the value function using the natural policy gradient (NPG) algorithm. 

\begin{definition}[Softmax Parameterization]
% \donghao{Need to separate the definition of softmax parameterization and other contents.}
Under the tabular MDP setting, the policy follows a softmax parameterization, where the policy \(\pi\) is parameterized by \(\theta : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}\). The policy is expressed as $\pi(a \vert s) = \frac{\exp(\theta(s, a))}{\sum_{a^{\prime} \in \mathcal{A}} \exp(\theta(s, a^{\prime}))}$.
\end{definition}
Policy improvement is performed using the natural policy gradient method \citep{kakade2002approximately}, where the policy parameter \(\theta\) is updated as $  \theta \leftarrow \theta + \eta \big(\mathcal{F}^{\theta}_{\rho}\big)^{\dagger} \nabla_{\theta} V^{\pi}(\rho)$ at each iteration, where $\mathcal{F}^{\theta}_{\rho} = \mathbb{E}_{s \sim \rho, a \sim \pi} \big[\nabla_{\theta} \log \pi_{\theta}(a \vert s) \nabla_{\theta} \log \pi_{\theta}(a \vert s)^\top\big]$ denotes the Fisher information matrix, 
and the \(\dagger\) operator denotes the Moore-Penrose inverse. Based on this setup, we now present the convergence guarantees.

\begin{theorem}\label{main thm}
Let \(\Tilde{\pi}\) be the weighted policy obtained after \(T\) iterations of Algorithm \ref{alg: main algo} with proper step-sizes.
Suppose that the offline dataset has a size of \(|\mathcal{D}^{\mu}| = \mathcal{O}\big(\frac{C \ln({|\mathcal{F}|}/{\delta})}{\epsilon_{\text{offline}} (1-\gamma)^4}\big)\) for some \(\delta \in (0, 1)\), where \(\mathcal{F}\) represents the critic function family.
Then,  with probability \(\geq 1 - \delta\), the optimality gap and constraint violation satisfy that
\begin{equation}
     V^{\pi_{\theta^*}}_r\hspace{-1pt}(\rho) \hspace{-2pt}-\hspace{-2pt} \mathbb{E}[V^{\Tilde{\pi}}_r(\rho)] \hspace{-1pt}\leq\hspace{-1pt} \mathcal{O}(\epsilon_{\text{offline}})\hspace{-1pt}+\hspace{-1pt}\mathcal{O}\hspace{-2pt}\left(\hspace{-2pt}\sqrt{\frac{|\mathcal{S}||\mathcal{A}|}{(1-\gamma)^3T}}\right)\hspace{-2pt},\hspace{-2pt}\label{reward bound}
\end{equation}
\begin{equation}
     \mathbb{E}[V^{\Tilde{\pi}}_c(\rho)] - b \leq \mathcal{O}(\epsilon_{\text{offline}}) + \mathcal{O}\left(\sqrt{\frac{|\mathcal{S}||\mathcal{A}|}{(1-\gamma)^3T}}\right),\label{cost bound}
\end{equation}
% \begin{equation}
%     \begin{aligned}
%         V^{\pi_{\theta^*}}_r(\rho) - \mathbb{E}[V^{\Tilde{\pi}}_r(\rho)] &\leq \mathcal{O}\left(\sqrt{\frac{|\mathcal{S}||\mathcal{A}|}{(1-\gamma)^3T}}\right), \\
%         \mathbb{E}[V^{\Tilde{\pi}}_c(\rho)] - b &\leq \mathcal{O}(\epsilon_{\text{offline}}) + \mathcal{O}\left(\sqrt{\frac{|\mathcal{S}||\mathcal{A}|}{(1-\gamma)^3T}}\right),
%     \end{aligned}
%     \label{main thm eq}
% \end{equation}
where $\epsilon_{\text{offline}}$ denotes the approximation error of policy evaluation induced by the offline dataset $\mathcal{D}^\mu$.
\end{theorem}
% \donghao{Mention that we will specify the definition of the weighted policy in the proof/appendix.}
For simplicity, we drop the reverse KL term to ensure the policy's closed-form update under NPG in our proof. 
The SafeAdaptation step in Algorithm \ref{alg: main algo} is  specified in algorithm \ref{alg: Safe Adapt} given in Appendix \ref{algo extension}. We specify the definition of the weighted policy $\Tilde{\pi}$ in Eq.~(\ref{defn: weighted policy}) given in Appendix \ref{proof of main thm}. We can interpret the theorem as follows: by selecting appropriate slack bounds $h^+$ and $h^-$, the policy optimization process will, over time, primarily remain in the reward optimization and gradient manipulation stages. As a result, the cost violation can be effectively upper bounded. Simultaneously, by ensuring that the policy is updated using the reward critic's gradients for the majority of iterations, we can guarantee that the accumulated reward of the weighted policy closely approximates that of the optimal policy. 

    
